Local and Distributed Quantum Computation

Experimental groups are now fabricating quantum processors powerful enough to execute small instances of quantum algorithms and definitively demonstrate quantum error correction that extends the lifetime of quantum data, adding urgency to architectural investigations. Although other options continue to be explored, effort is coalescing around topological coding models as the most practical implementation option for error correction on realizable microarchitectures. Scalability concerns have also motivated architects to propose distributed memory multicomputer architectures, with experimental efforts demonstrating some of the basic building blocks to make such designs possible. We compile the latest results from a variety of different systems aiming at the construction of a scalable quantum computer.

==> Makefile <==
.SUFFIXES: .pdf .xbb .tex .cls
.pdf.xbb:; extractbb $<

TEX = ieee-computer-survey.tex introduction.tex quantum-concepts.tex \
	divincenzo.tex \
	architectures.tex experimental-progress.tex \
	software-control.tex networks.tex conclusions.tex
XBB = 
BIB = paper-reviews.bib ieee.bib
FIGS = generations.jpeg offline.jpeg online.jpeg surface.jpeg
TEXENV = TEXINPUTS="./revtex:${TEXINPUTS}"; export TEXINPUTS; 
LTXCMD=pdflatex
all: ieee-computer-survey.pdf


ieee-computer-survey.pdf: ${TEX} ${XBB} ${BIB} ${FIGS}
	${TEXENV} ${LTXCMD} ieee-computer-survey.tex
	${TEXENV} bibtex ieee-computer-survey
	${TEXENV} ${LTXCMD} ieee-computer-survey.tex
	${TEXENV} ${LTXCMD} ieee-computer-survey.tex

# ieee-computer-survey.pdf: ieee-computer-survey.dvi
#	dvipdf ieee-computer-survey

count:
	texcount ${TEX}

clean::
	/bin/rm -f ieee-computer-survey.aux ieee-computer-survey.blg ieee-computer-survey.dvi ieee-computer-survey.log ieee-computer-survey.out

realclean:: clean
	/bin/rm -f ieee-computer-survey.pdf

